TARGET: Automated Scenario Generation from Traffic Rules for Testing Autonomous Vehicles via Validated LLM-Guided Knowledge Extraction

Recent incidents with autonomous vehicles highlight the need for rigorous testing to ensure safety and robustness. Constructing test scenarios for autonomous driving systems (ADSs), however, is labor-intensive. We propose TARGET, an end-to-end framework that automatically generates test scenarios from traffic rules. To address complexity, we leverage a Large Language Model (LLM) to extract knowledge from traffic rules. To mitigate hallucinations caused by large context during input processing, we introduce a domain-specific language (DSL) designed to be syntactically simple and compositional. This design allows the LLM to learn and generate test scenarios in a modular manner while enabling syntactic and semantic validation for each component. Based on these validated representations, TARGET synthesizes executable scripts to render scenarios in simulation. Evaluated seven ADSs with 284 scenarios derived from 54 traffic rules, TARGET uncovered 610 rule violations, collisions, and other issues. For each violation, TARGET generates scenario recordings and detailed logs, aiding root cause analysis. Two identified issues were confirmed by ADS developers: one linked to an existing bug report and the other to limited ADS functionality.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> paper/method/generator_2.tex <==
\subsection{Template-based Test Script Generation}
\label{sec:generator}
%In this study, we propose a template-based scenario generation method. For a simulator, we first create a template scenario\jz{script} that defines the running procedure of a test scenario based on the simulator APIs.
% \tocheckjz{In this research, we introduce a method for scenario generation based on templates. For a given simulator, we begin by crafting a template script, outlining the execution process of a test scenario using the simulator's APIs, as shown in Listing~\ref{lst:template_script}.
% Using this template script, we simply associate each function within it with the respective subcomponent and substitute function parameters with elements from the corresponding subcomponents in the scenario representation.} 
%}

After the functional scenario description is generated by the rule parser, it is then used to construct a concrete scenario that can run in simulators. Inspired by templated-based code generation~\cite{jorges2013state}, we propose a template-based test script generation method to do this. We first create a \textit{template script} that outlines the core functions required to execute a test scenario using the simulator's APIs, as shown in Listing~\ref{lst:template_script}. {\color{black}The values of key parameters including \textit{weather parameter}, \textit{time parameter}, \textit{ego\_initial\_coordiate}, \textit{npc\_initial\_coordinate}, \textit{ego\_destination\_coordinate}, \textit{npc\_destination\_coordinate}, \textit{longitudinal oracle}, and \textit{lateral oracle} need to be determined by the scenario generator based on the test scenario representation and data obtained from the simulator. We propose \textit{dictionary search} and \textit{Hierarchical Map-based Route Search} to identify the parameter values. The overall process is shown in Algorithm~\ref{alg:param}.

% Once the test scenario representation is obtained, the key challenge is to convert the abstract scenario representation to a concrete, executable scripts in a simulator.
% Inspired from templated-based code generation~\cite{jorges2013state}, we propose a template-based test script generation method to do this. We first create a \textit{template script} that outlines the core functions required to execute a test scenario using the simulator's APIs, as shown in Listing~\ref{lst:template_script}. Once the parameters \textit{weather parameter}, \textit{time parameter}, \textit{ego\_initial\_coordiate}, \textit{npc\_initial\_coordinate}, \textit{ego\_destination\_coordinate}, \textit{npc\_destination\_coordinate}, \textit{longitudinal oracle}, and \textit{lateral oracle} of the core functions in the template script have been determined, an executable test script is generated. To determine the concrete parameters, we propose \textit{dictionary search} and \textit{Hierarchical Map-based Route Search} to deal with different components in the dictionary-format scenario representation as shown in Figure~\ref{fig:example_scenario_dsl}.




% Our proposed method for generating executable test scripts draws inspiration from template-based code generation techniques. This approach allows us to efficiently convert abstract test scenario representations into concrete, executable scripts tailored to specific simulation environments.


% Once the test scenario representation is obtained, it should be converted to the executable test script to render the corresponding test scenario in the simulation. In our research, we propose a template-based method for test script generation. For a specific simulator, we create a template script that details the test scenario's execution using the simulator's APIs in Listing~\ref{lst:template_script}. We then link each function in the script to its relevant subcomponent in the scenario representation and identify specific function parameters by the corresponding subcomponent elements.



\begin{lstlisting}[language=Python, caption=Simplified template scenario script,label={lst:template_script},captionpos=b]
def run_scenario(*args):
    set_environment(weather_params, time_params)
    set_actors(ego_initial_coordinate, 
               ego_destination_coordinate,
               npc_initial_coordinate, 
               npc_destination_coordinate)
    set_test_oracle(longitudinal_oracle, 
                    lateral_oracle)

def set_environment(weather_params, time_params):
    simulator.set_weather(weather_params)
    simulator.set_time(time_params)

def set_actors(ego_initial_coordinate, 
               ego_destination_coordinate,
               npc_initial_coordinate, 
               npc_destination_coordinate):
    simulator.set_actor_position(ego_vehicle, 
                      ego_initial_coordinate)
    ads.move_to(ego_destination_coordinate)
    
    simulator.set_actor_position(npc_actor, 
                    npc_initial_coordinate)
    simulator.move_npc_to(npc_actor,
                npc_destination_coordinate)

def set_test_oracle(longitudinal_oracle,
                            lateral_oracle):
    monitor.set_oracles(longitudinal_oracle,
                             lateral_oracle)

 \end{lstlisting}


\begin{algorithm*}
\SetAlgoLined
\SetKwInput{Input}{Input~}
\SetKwInput{Output}{Output~}
    \SetKwData{Scenario}{SP}
    \SetKwData{ParamDict}{PD}
    \SetKwData{Params}{PV} 
    \SetKwData{MapInfo}{MapInfo} 
    \SetKwData{Simulator}{Simulator} 
    \SetKwData{Route}{Route}
    \SetKwData{Routes}{Routes}
    \SetKwData{QR}{QR}
    \SetKwData{NearbyRoutes}{NearbyRoutes}
    \SetKwData{EgoRoutes}{EgoRoutes}
    \SetKwData{EgoRoute}{EgoRoute}
    \SetKwData{NPCRoute}{NPCRoute}
    \SetKwData{Flag}{Flag}
    
    \SetKwFunction{GetMapInfo}{GetMapInfo}
    \SetKwFunction{GetRoutes}{GetRoutes}
    \SetKwFunction{Waypoints}{Waypoints}
    \SetKwFunction{GetPrevRoute}{GetPrevRoute}
    \SetKwFunction{FilterRouteByRoadNetwork}
    {FilterRouteByRoadNetwork}
    \SetKwFunction{Append}{append}
    \SetKwFunction{FilterRouteByActor}{FilterRouteByActor}
    \SetKwFunction{SampleWaypoints}{SampleWaypoints}
    \SetKwFunction{CheckEgoRoute}{CheckEgoRoute}
    \SetKwFunction{CheckNPCRoute}{CheckNPCRoute}
    \SetKwFunction{GetNearbyRoutes}{GetNearbyRoutes}
    
    
    \Input{\Scenario: test scenario representation in dictionary format; \ParamDict: Lookup table of parameter values for subcomponents Environment and Oracle}
    \Output{\Params: dictionary of parameter values}
    \ccomment{ \tcc{Get parameter values for parameters weather\_params, time\_params, longitudinal\_oracle, and lateral\_oracle by dictionary search}}
    \Params[``weather''] $\leftarrow$ \{\Scenario[``Environment''][``Weather'']\; \ParamDict[\Scenario[``Environment''][``Weather'']]\}\; 
    \Params[``time''] $\leftarrow$ \ParamDict[\Scenario[``Environment''][``Time'']]\;
    \Params[``longitudinal\_oracle''] $\leftarrow$ \ParamDict[\Scenario[``Oracle''][``longitudinal\_oracle'']]\;
    \Params[``lateral\_oracle''] $\leftarrow$ \ParamDict[\Scenario[``Oracle''][``lateral\_oracle'']]\;        
    
    \ccomment{\tcc{Initialize \Routes and \QR to save all routes and filtered routes that match \Scenario[``Road\_network'']}}
    \Routes $\leftarrow$ []\;
    \QR $\leftarrow$ []\ ;
    \MapInfo $\leftarrow$ \GetMapInfo(\Simulator)\;
    \Waypoints $\leftarrow$ \SampleWaypoints(\Simulator)\;
    \Routes $\leftarrow$ \GetRoutes(\Waypoints, \MapInfo)\;
    
    \ForEach {\Route $\in$ \Routes}{%
        \If {\FilterRouteByRoadNetwork(\Route, \Scenario[``Road\_network''])}{
            \QR.\Append{\Route}\;
        }
    }

    \ForEach {\Route $\in$ \QR}{%
        \If {\FilterRouteByActor(\Route, \Scenario[``Actors''][``ego\_vehicle''])}{
            \EgoRoutes.\Append{\Route}\;
        }
    }
    
    \ForEach {\Route $\in$ \EgoRoutes}{%
        \NearbyRoutes $\leftarrow$ \GetNearbyRoutes(\Route)\;
        \ForEach {\NPCRoute $\in$ \NearbyRoutes}{
            \If {\FilterRouteByActor(\NPCRoute, \Scenario[``Actors''][``other\_actors''])}{
                \Flag $\leftarrow$ \textsf{true}\;
                \textsf{break}\;
            }            
        }
        \If {\Flag}{
            \textsf{break}\;
        }
    }
    
    \ccomment{ \tcc{Get parameter values for parameters ego\_initial\_coordinate, ego\_destination\_coordinate, npc\_initial\_coordinate, npc\_destination\_coordinate}}
    \If {\Flag}{
        \Params[``ego\_initial\_coordinate''] $\leftarrow$ \GetPrevRoute(\EgoRoute).start\_point\;
        \Params[``ego\_destination\_coordinate''] $\leftarrow$ \EgoRoute.end\_point\;
        \Params[``npc\_initial\_coordinate''] $\leftarrow$ \NPCRoute.start\_point\;
        \Params[``npc\_destination\_coordinate''] $\leftarrow$ \NPCRoute.end\_point\;
        
    }
    
\caption{Scenario Parameter Identification}
\label{alg:param}
\end{algorithm*}
 % Listing~\ref{lst:template_script} shows a simplified template test script that contains four key functions to generate a test scenario by the simulator. To make it as an executable test script, the placeholder function paramters \textit{weather parameter}, \textit{time parameter}, \textit{ego\_initial\_coordiate}, \textit{npc\_initial\_coordinate}, \textit{ego\_destination\_coordinate}, \textit{npc\_destination\_coordinate}, \textit{longitudinal oracle}, and \textit{lateral oracle} need to be filled. 
 
 % The function \texttt{set\_environment} invokes simulator APIs to set the weather and time of the test scenario based on \textit{weather parameter} and \textit{time parameter}. In the function \texttt{set\_actors}, the ego vehicle and the NPC actor are created on \textit{ego\_initial\_coordiate} and \textit{npc\_initial\_coordinate} respectively. Then, the ADS under test controls the ego vehicle to move to \textit{ego\_destination\_coordinate} and the simulator controls the NPC to move to \textit{npc\_destination\_coordinate}. The function \texttt{set\_test\_oracle} feeds \textit{longitudinal oracle} and \textit{lateral oracle} to the scenario monitor to check the erroneous behaviors of the ADS under test, which will be introduced in Section~\ref{sec:test_monitor}.

%  Given a scenario representation, the test script generator first converts it to a dictionary containing key-value pairs based on the DSL syntax in Figure~\ref{fig:schema}. For each key-value pair, the key is the name of the subcomponent (left-hand side) defined in the DSL  and the value is the corresponding element (right-hand side in the DSL) in the scenario representation. Then, the key-value pairs are used to identify concrete parameters of the given functions in the template script.
% Considering the link between required function parameters and elements in the scenario representation, we have two approaches to set these parameters: the dictionary search method and an approach using a hierarchical map-based route-search algorithm, as detailed further below.

\subsubsection{Dictionary Search} 
Lines 2-5 in Algorithm~\ref{alg:param} show how to obtain parameter values for  weather\_params, time\_params, longitudinal\_oracle, and lateral\_oracle through a dictionary search. A lookup dictionary \texttt{PD} is created in advance that maps from the subcomponent value in the test scenario representation to the parameter value in the simulation. For example, for the simulator Carla, a default parameter and its value ``fog\_density: 0.5'' is stored in the field ``foggy'' in \texttt{PD}. Once the value ``foggy'' is found from the test scenario presentation subcomponent \textit{SP[``Environment''][``Weather'']}, the parameter value weather\_param for the function set\_environment in the template scenario script is set. A similar process is applied for other parameters about time and oracle.


% For functions \texttt{set\_environment} and \texttt{set\_test\_oracle}, the function parameters are identified by dictionary search.

% \label{concrete_function_Direct}
% \textbf{Set Environment}: By iterating the key-value dictionary, the test script generator uses the key to identify the function parameter and uses the value to identify the corresponding parameter value.} 
% For example, when retrieving the key-value pair \textit{\{``weather'': ``foggy''\}}, the key \textit{``weather''} corresponds to the function parameter \textit{weather\_params}.
% Once the function parameter is found, the value ``foggy'' is used to set the value for \textit{weather\_params}. For a given simulator, we devised an internal mapping for each environment condition such as foggy and rainy. For instance, if the simulator is Carla, ``foggy'' corresponds to the ``fog\_density'' setting. By default, this sets \textit{weather\_params} to ``fog\_density = 0.5'' in Carla. Future work will delve into exploring the environmental condition value space to pinpoint corner cases that breach traffic rules.

% {\color{blue}\textbf{Set Test Oracle}: When retrieving key-value pairs, once the keys \textit{``longitudinal\_oracle''} and \textit{``lateral\_oracle''} are identified, their corresponding values, such as \textit{decelerate} and \textit{keep\_lane}, are obtained and directly fed to the template function \texttt{set\_test\_oracle} to set the scenario monitor.}

\subsubsection{Hierarchical Map-based Route search} 
\label{concrete_function_Search} 
To obtain the parameter values of accurate coordinates for the ego vehicle and NPC actors, we propose a hierarchical map-based route-search algorithm in the test script generator following steps \textit{Routes Generation}, \textit{Route filter}, \textit{Ego Route identification}, and \textit{Actors coordinate identification}, as shown in Lines 8 to 40 in Algorithm~\ref{alg:param}.

\textbf{Routes Generation}: The test script generator initially acquires comprehensive map information from the simulator, including the waypoints (coordinates) of the start and end points of each lane and the waypoints of all traffic signs. Subsequently, the scenario script generator implements a uniform sampling algorithm to extract waypoints along all lanes within the map. \textit{Routes} are then constructed by establishing connections between adjacent sampled waypoints along each lane, as illustrated in Figure~\ref{fig:route_scenario} (a). For each generated \textit{route}, a set of salient attributes is computed based on the acquired map information, including route length, route direction, the connecting routes at the start or end waypoints, and the presence of traffic signs on the route, and whether the route traverses an intersection or other types of road are calculated based on the map information. For example, the route from E to C in Figure~\ref{fig:route_scenario} (b) may contain information that the start waypoint be (5, 5); the end waypoint be (5, 10); the route direction be straight.

% The test script generator first obtains \textit{Waypoints} (coordinates) and \textit{routes} information from the simulator map that is used to generate the test scenario. Specifically, waypoints on all roads in the simulation map are directly obtained by calling the corresponding simulator API, such as \texttt{get\_waypoints} in Carla. Then, \textit{routes} are created by connecting two adjacent waypoints along a road lane, as shown in Figure~\ref{fig:route_scenario} (a). Moreover, route-related information such as length, direction, the connecting routes at the start or end waypoints, the presence of traffic signs on the route, and whether the route traverses an intersection or other types of road are retrieved based on the map information in the simulator. 

\textbf{Route Filter}: With all \textit{Routes}, the test script generator filters all qualified routes into the list \texttt{QR} based on key-value pairs of the Road Network subcomponents in the test scenario representation. For example, given key-value pairs such as \textit{``road type'': ``intersection'', ``road marker'': ``solid line'', ``traffic signs'': [``speed limit sign'']}, \texttt{QR} is created to contain all routes featuring solid line boundaries, intersecting an intersection, and incorporating a speed limit sign.

% Based on the key-value pairs of \textit{Road network} subcomponents, the test script generator iteratively checks whether each route contains corresponding subcomponent elements and saves qualified routes in a route list. For example, if the key-value pairs \textit{``road type'': ``intersection'', ``road marker'': ``solid line'', ``traffic signs'': [``speed limit sign'']} is obtained, the test script generator will find all routes that contain solid line and pass through an intersection and a speed limit sign into a route list. The route list is then used to identify the potential ego route to set up the ego vehicle.

\textbf{Ego Route Identification}: The generated route list \texttt{QR} undergoes further analysis to determine eligible routes for the ego vehicle, based on key-value pairs of \textit{ego vehicle} subcomponents. For example, if the key-value pairs are \textit{``behavior'': ``go forward'', ``position reference'': ``intersection'', ``position relation'': ``behind''}, the route that drives straight through an intersection is identified as a potential \texttt{ego route}. This process yields a set of candidate ego routes \texttt{EgoRoutes} as shown in Algorithm~\ref{alg:param} Lines 18 to 22, for subsequent NPC route identification.
 
\textbf{NPC Route Identification}: As shown in Algorithm~\ref{alg:param} Lines 23 to 34, the test script generator iterates all ego route candidates in \texttt{EgoRoutes}. For each ego route candidate, the test script generator checks whether its nearby routes meet the requirements for each \textit{NPC actor} subcomponent  (e.g., another route for moving forward and crossing with the go route candidate). If the eligible NPC routes can be found near the ego route candidate, both \texttt{ego route} and \texttt{NPC routes} are formally identified. The iteration is then terminated. If no valid combination of ego and NPC routes can be established after an exhaustive evaluation of all ego route candidates, the test script generator declares the scenario infeasible for generation on the current simulation map.

% Once a potential ego route is identified, the test script generator further checks its nearby routes to identify the NPC routes that meet the requirements of key-value pairs for each \textit{NPC actor} subcomponent (e.g., another route for going forward and crossing with the \texttt{ego route}). If the eligible NPC routes can be found near the potential ego route, both \texttt{ego route} and \texttt{NPC routes} are formally identified. Otherwise, the identification process for NPC routes is iteratively implemented on all potential \texttt{ego route}. If suitable NPC routes are located in the vicinity of a potential ego route, both the ego and NPC routes are formally designated. In the absence of viable NPC routes, the identification process is iteratively applied to all potential ego routes within the route list. If no valid combination of ego and NPC routes can be established after exhaustive evaluation of all potential ego routes, the test script generator declares the scenario infeasible for generation on the current simulation map.
  
\textbf{Actors Coordinate Identification}:
Once \texttt{ego route} and the \texttt{NPC routes} are identified, the parameter value of ego\_initial\_coordinate is set at the start waypoint of the previous connecting route to the ego route, enabling the ADS to accelerate to a steady speed before achieving the start waypoint of the identified ego route (e.g., the entrance of an intersection) of the test scenario.  The ego\_destination\_coordinate is set as the end waypoint of the ego route. The initial points and destinations for other actors are the start and the end waypoints of their respective routes. An example can be found in Figure~\ref{fig:route_scenario} (b).

{\color{blue}\textbf{Executable Script Formation}}

% The ego vehicle's initial position is set at the start waypoint of the previous connecting route to the ego route, enabling the ADS to accelerate to a steady speed before achieving the  start waypoint of the identified ego route (e.g., the entrance of an intersection) of the test scenario. The ego vehicle's destination is set as the end waypoint of the ego route.  Initial points and destinations for other actors are the start and the end waypoints of their respective routes. An example can be found in Figure~\ref{fig:route_scenario} (b). When all coordinates are identified, they are fed to the template function \texttt{set\_actors}.


% \tz{When reading here, it occurred to me that the current split of this section (template scenario generator and concrete scenario generator) is not very good. You should give a more detailed breakdown. This paragraph definitely talks about something non-trivial and deserve to have a subsection header.}The constraints of the road network and actors are converted to \textit{Waypoints} (coordinates) of the initial positions and destinations of the ego vehicle and NPC actors for controlling their movements. To do this, the scenario generator first constructs \textit{Routes} based on the map information provided by the simulator.
% The conversion is based on the map information provided by the simulator. Specifically, the scenario generator obtains the information of \textit{Waypoints} 
% employs data structures \textit{Waypoint} and \textit{Route} to represent map information from the simulator. 
% A Waypoint is a coordinate of a point on a road line on the map,  while 

% a \textit{route} defines a trajectory from one waypoint to the adjacent waypoint along the road lane, as shown in Figure~\ref{fig:route_scenario} (a). Moreover, a \textit{route} also contains attributes such as length, direction, the presence of traffic signs on the route, and whether the route traverses an intersection. Leveraging the route information, the scenario generator identifies a list of routes that satisfy the constraints of the road network (e.g., \texttt{road type, is, intersection}).

% The scenario generator then iterates over each route in the candidate route list. If a route meets the constraints of the ego vehicle, it is designated as the ego route. Subsequently, the generator iterates over the neighboring routes of the ego route to check whether they fulfill the constraints of other actors, thereby generating a list of NPC routes. The iteration process ends once a combination of the ego route and NPC routes that satisfy all constraints for the ego vehicle and other actors is found. The parameters for the initial and destination positions of all actors are then identified based on the established ego route and NPC routes. The ego vehicle's initial position is set at the starting point of the previous route to the ego route, enabling the ADS to accelerate to a steady speed before achieving the trigger point of the test scenario. The ego vehicle's destination is set as the end waypoint of the ego route.  Initial points and destinations for other actors are the start and the end waypoints of their respective routes. An example can be found in Figure~\ref{fig:route_scenario} (b).

% When API invocations and parameters for all functions are identified, the concrete scenario script is formed for rendering the corresponding scenario.

% Based on the selected routes and the constraints of actors, The scenario generator determines accurate parameters including the initial positions and destinations of actors) for the ego vehicle and other actors. It verifies each route for its compatibility with the behavior constraint, such as turning left, of the ego vehicle. For the eligible route, the generator checks whether adjacent routes of the eligible route meet the requirements of other actors. When the first combinations of routes eligible for all actor constraints are established, the accurate parameters for all actors can be identified. Specifically, the ego vehicle's initial position is set at the starting point of the predecessor route to the ego route, allowing the ADS to reach a steady speed before the test scenario begins. The ego vehicle's destination is the endpoint of the ego route. Spawn points and destinations for other actors are linked directly to their respective routes. An example can be found in Figure~\ref{fig:route_scenario} (b).

% For test oracles, the scenario generator integrates the corresponding test oracle API in accordance with the constraints. For some test orcale APIs, parameters are derived from traffic rule handbooks~\cite{texasDriverHandbook}, such as 3-second safety distance for the longitudinal oracle \textit{keep distance}. In addition, some parameters are derived from the map information. For example, the test oracle \textit{decelerate} checks whether the speed of the ego vehicle decelerates to less than the speed limit specified on the speed limit sign on the road.




% Speed limits are evaluated either by road signs or, in their absence, by comparing average speeds over the route halves. A safe driving distance is maintained using a predefined 3-second parameter from driver handbooks.

% For test oracles, the scenario generator incorporates the corresponding test oracle API such as \texttt{stop}, \texttt{decelerate}, \texttt{keep distance}, and \texttt{keep lane}, according to the constraints. The parameters of the are drawn from traffic rule handbooks~\cite{texasDriverHandbook} and  Speed limits are evaluated either by road signs or, if absent, by comparing average speeds over the route halves. Safe driving distance is maintained using a predefined 3-second parameter from driver handbooks. 
% \\
% \\
% When the four components are constructed, the scenario generator combines them to create the scenario script that can be loaded by the simulator to render the corresponding scenario.

% \subsubsection{Environment Creation}
% Based on elements in the field \textit{Environment} of the scenario representation, the scenario generator invokes corresponding simulator APIs to define the weather in the driving environment. As our DSL does not allow users to define parameters due to the aim of keeping the simple way to describe test scenarios, in the current work, all parameters are assigned as default values. For environment parameters such as \texttt{fog}, the parameter is set as 0.5. In future work, we will explore the parameter space using search-based methods to create more diverse test scenarios in accordance with traffic rule descriptions.

% On the other hand, the scenario generator also controls traffic signals within the simulator. If words related to ``traffic light'' is mentioned in the scenario representation, the scenario generator ensures that the traffic light is in the corresponding status (e.g., red) when the ego vehicle approaches it.


% \begin{figure}[tb!]
% \centering
% \includegraphics[width = .7\textwidth]{image/scenario_example_.pdf}
% \caption{The demonstration of waypoints, routes, and a driving scenario}
% \label{fig:route_scenario}
% \end{figure}


\begin{figure}[tb!]
\centering
\includegraphics[width = .5\textwidth]{image/road.pdf}
\caption{The demonstration of waypoints, routes, and a driving scenario}
\label{fig:route_scenario}
\end{figure}

% \subsubsection{Scenario Location Identification}
% Leveraging on the map information provided by the simulator and elements in the scenario representation, the scenario generator identifies all locations where the test scenario possibly occurs. Specifically, the generator samples waypoints on all lanes in the map and forms routes by connecting adjacent waypoints, as examples shown in Figure~\ref{fig:route_scenario} (a). For each route, its attributes such as length, direction, and whether it crosses an intersection are calculated based on the map information. Then, the generator applies enumerative search to select routes that match the \textit{Road network} elements in the scenario representation, such as selecting all routes that cross an intersection when the element \texttt{intersection} is specified in the \textit{Road network} field.

% During the enumerative search process of routes, the generator also identifies whether the current route is compatible with the behavioral requirements (e.g., turn left) of the ego vehicle and other actors. 

% Based on the selected routes, The scenario generator determines accurate spawn points (i.e., the initial positions of actors) and destinations for both the ego vehicle and other actors based on a depth-first search. It verifies each route for its compatibility with the behavioral requirements of the ego vehicle defined in the scenario representation, like turning left. For the eligible route, the generator checks whether adjacent routes of the eligible route meet the requirements of other actors. When the first combinations of routes eligible for all actors are established, the search process ends, and the generator assigns spawn points and destinations for all actors. The ego vehicle's spawn point is set at the starting point of the predecessor route to the ego route, allowing the ADS to reach a steady speed before the test scenario begins. The ego vehicle's destination is the endpoint of the ego route. Spawn points and destinations for other actors are linked directly to their respective routes. An example can be found in Figure~\ref{fig:route_scenario} (b).


% \subsubsection{Test Oracle Creation}
% \label{sec:test_criteria}
% The scenario generator incorporates various oracle options to determine the expected ego vehicle behavior, such as \texttt{yield}, \texttt{stop}, \texttt{decelerate}, \texttt{keep distance}, and \texttt{keep lane}, according to elements in the field \texttt{Oracle} in the scenario representation. These options, drawn from traffic rule handbooks~\cite{texasDriverHandbook} and OpenXOntology~\cite{openxontology}, assess adherence to right-of-way rules, traffic signs, speed limits, safe driving distances, and lane maintenance. Speed limits are evaluated either by road signs or, if absent, by comparing average speeds over the route halves. Safe driving distance is maintained using a predefined 3-second parameter from driver handbooks. 
% \\
% \\
% When the four components are constructed, the scenario generator combines them to create the scenario script that can be loaded by the simulator to render the corresponding scenario.


==> paper/method/scenario_generator.tex <==
\subsection{Template-based Test Script Generation}
\label{sec:generator}
%In this study, we propose a template-based scenario generation method. For a simulator, we first create a template scenario\jz{script} that defines the running procedure of a test scenario based on the simulator APIs.
% \tocheckjz{In this research, we introduce a method for scenario generation based on templates. For a given simulator, we begin by crafting a template script, outlining the execution process of a test scenario using the simulator's APIs, as shown in Listing~\ref{lst:template_script}.
% Using this template script, we simply associate each function within it with the respective subcomponent and substitute function parameters with elements from the corresponding subcomponents in the scenario representation.} 
%}



Once the test scenario representation is obtained, it should be converted to the executable test script to render the corresponding test scenario in the simulation. In our research, we propose a template-based method for test script generation. For a specific simulator, we create a template script that details the test scenario's execution using the simulator's APIs in Listing~\ref{lst:template_script}. We then link each function in the script to its relevant subcomponent in the scenario representation and identify specific function parameters by the corresponding subcomponent elements.


%Based on the scenario representation, the key parameters and their values of the invoked simulator APIs are identified to form the concrete test scenario. 

% Based on the formal scenario representation, the scenario generator implements the program synthesis~\cite{gulwani2017program, manna1971toward} process to create a scenario script that defines a runnable concrete test scenario in simulation. Specifically, the scenario generator applies components-based synthesis~\cite{gulwani2017program} to decouple the scenario script into four functions: 

% Upon acquiring the scenario representation, the objective of the scenario generator is to construct a test scenario script capable of being loaded by a simulator to render a concrete test scenario. Given the scenario representation, it first creates a template scenario script \tz{Where are the templates from? Manually defined? Based on what? Need to provide a brief description here.}with template scenario functions. The template functions contain function constraints to describe the requirements for the function within the concrete scenario script. The function constraints are then solved and converted to actual API invocations and API parameters in the concrete scenario functions.

% To achieve this, the scenario generator initially creates a template scenario script that defines the requisite functions for the simulator to render the scenario. Subsequently, the scenario generator identifies specific parameters within each function to formulate the concrete test scenario script.

% In the template scenario script, the functions do not contain specific parameters 
% to control the weather, the road network location where the driving scenario occurs, the behaviors of all actors, and the test oracles for ADS performance evaluation. 

% The test scenario script is composed of four functions: a) Control the environment in the driving scenario; b) Identify the initial locations of all actors where the driving scenario occurs in the simulator map; c) Define all actors' behaviors in the driving scenario; d) Create test oracles to check whether the ego vehicle has erroneous behaviors such as traffic rule violations and collisions. 

% The scenario generator follows three steps to construct the test scenario script. First, it parses the input scenario representation as \textit{constraints} represented in triplet turples. Then, it extracts the map information and generates \textit{routes}, which are used to solve constraints of the road network and actors. Finally, it constructs four functions with concrete parameters by solving all constraints, and generate the test scenario script.

%\subsubsection{Template Scenario}

\begin{lstlisting}[language=Python, caption=Simplified template scenario script,label={lst:template_script},captionpos=b]
def run_scenario(*args):
    set_environment(weather_params, time_params)
    set_actors(ego_initial_coordinate, 
               ego_destination_coordinate,
               npc_initial_coordinate, 
               npc_destination_coordinate)
    set_test_oracle(longitudinal_oracle, 
                    lateral_oracle)

def set_environment(weather_params, time_params):
    simulator.set_weather(weather_params)
    simulator.set_time(time_params)

def set_actors(ego_initial_coordinate, 
               ego_destination_coordinate,
               npc_initial_coordinate, 
               npc_destination_coordinate):
    simulator.set_actor_position(ego_vehicle, 
                      ego_initial_coordinate)
    ads.move_to(ego_destination_coordinate)
    
    simulator.set_actor_position(npc_actor, 
                    npc_initial_coordinate)
    simulator.move_npc_to(npc_actor,
                npc_destination_coordinate)

def set_test_oracle(longitudinal_oracle,
                            lateral_oracle):
    monitor.set_oracles(longitudinal_oracle,
                             lateral_oracle)

 \end{lstlisting}
 
 Listing~\ref{lst:template_script} shows a simplified template test script that contains four key functions to generate a test scenario by the simulator. The function \texttt{set\_environment} invokes simulator APIs to set the weather and time of the test scenario based on \textit{weather parameter} and \textit{time parameter}. In the function \texttt{set\_actors}, the ego vehicle and the NPC actor are created on \textit{ego\_initial\_coordiate} and \textit{npc\_initial\_coordinate} respectively. Then, the ADS under test controls the ego vehicle to move to \textit{ego\_destination\_coordinate} and the simulator controls the NPC to move to \textit{npc\_destination\_coordinate}. The function \texttt{set\_test\_oracle} feeds \textit{longitudinal oracle} and \textit{lateral oracle} to the scenario monitor to check the erroneous behaviors of the ADS under test, which will be introduced in Section~\ref{sec:test_monitor}.

 Given a scenario representation, the test script generator first converts it to a dictionary containing key-value pairs based on the DSL syntax in Figure~\ref{fig:schema}. For each key-value pair, the key is the name of the subcomponent (left-hand side) defined in the DSL  and the value is the corresponding element (right-hand side in the DSL) in the scenario representation. Then, the key-value pairs are used to identify concrete parameters of the given functions in the template script.
Considering the link between required function parameters and elements in the scenario representation, we have two approaches to set these parameters: the dictionary search method and an approach using a hierarchical map-based route-search algorithm, as detailed further below.

\subsubsection{Dictionary Search} For functions \texttt{set\_environment} and \texttt{set\_test\_oracle}, the function parameters are identified by dictionary search.

\label{concrete_function_Direct}
\textbf{Set Environment}: By iterating the key-value dictionary, the test script generator uses the key to identify the function parameter and uses the value to identify the corresponding parameter value. 
For example, when retrieving the key-value pair \textit{\{``weather'': ``foggy''\}}, the key \textit{``weather''} corresponds to the function parameter \textit{weather\_params}.
Once the function parameter is found, the value ``foggy'' is used to set the value for \textit{weather\_params}. For a given simulator, we devised an internal mapping for each environment condition such as foggy and rainy. For instance, if the simulator is Carla, ``foggy'' corresponds to the ``fog\_density'' setting. By default, this sets \textit{weather\_params} to ``fog\_density = 0.5'' in Carla. Future work will delve into exploring the environmental condition value space to pinpoint corner cases that breach traffic rules.
%and the value \textit{``foggy''} is {\color{blue}mapped to the actual function parameter used in simulator APIs, such as \textit{``fog\_density''} in Carla. Once the function parameter is identified, it is set as the default value in the simulator (e.g., fog\_density=0.5). Future work will explore the parameter space using search-based methods to generate a more diverse array of test scenarios that align with traffic rule descriptions.
% mapped to \textit{``fog\_density''} in accordance to the simulator API signature

% \jz{no one understands API signagure. You basically use Weather to identify weatherParameter, this is easy to understand. how to map the value foggy to generate an instance of the weatherparams to setWeather is not easily understood. You need to mention there is a list of value acceptable by weatherParams, for instance fogDensity and give one more. Then if you retrieve the value Foggy, you have created a Simulator-Specific mapping function to map Foggy to FogDentisty. Now you also encounter another issue, that is you still need to set the value for fogDensity, in this implementation you need to highlight, you use the default value from the simulator. Your future work shall then follow, to talk about to search in this space to find corner cases where the setting of these environment elements such as foggyDensity and Sunxxxx will lead to violation of traffic rules.}. }

% for the subcomponents \textit{weather} and \textit{time}, the scenario generator maintains a parameter dictionary to map the subcomponent element to the corresponding parameter name used in the simulator API. The parameter dictionary has the structure \textsc{subcomponent element: [parameter name, default value]}. 
% For example, given the key-value pair \textsc{\{``weather'': ``foggy''\}}\jz{it is not consistent with your key value pair. I would suggest to change the data structure as normal just Key which is subcomponent element name, value is the element chosen. When you do the mapping, you use the subcomponent element name to find the function, and then identify the function parameter using the value in the dictionary. And then you mention in the Dictionary search, the value for each parameter will be set as the default one in the simulator. To be clear, the key-value pair is constructed from the scenario representation to identify the function and the parameter, while the value of the parameter, you have a heuristic, to set to a default value, largely from the simulator}, the element \texttt{foggy} of the subcomponent \textit{weather} maps to the parameter name \textsc{fog\_density} with a default value 0.5. Then, [fog\_density, 0.5] is fed as \textit{weather parameter} into the function \texttt{set\_weather}.

% In the proposed DSL we do not ask users to define the values for the parameters to keep the simple syntax. For instance, if it is foggy, we do not ask the user to specify how hard is the fog. Correspondingly, when converting these subcomponent elements to function parameters, we use default values to set them. Future work will explore the parameter space using search-based methods to generate a more diverse array of test scenarios that align with traffic rule descriptions\jz{This is very poorly written, change according to the commments above}.

% Based on the key-value pairs for the subcomponents \textit{weather} and \textit{time}, the scenario generator can directly retrieve the parameter name and its default value from a pre-defined parameter dictionary and then uses the parameter and value for the template function \texttt{set\_weather}. For example, given the key-value pair \textsc{\{``weather'': ``foggy''\}}, the corresponding parameter and value \textsc{fog\_density=0.5} is obtained and feed as \textit{weather parameter} into the function \texttt{set\_weather}.
% \jz{you need to do it step by step, firstly you need to mention with the key-value pairs, you can use the subcomponent name to identify the function, and then use the element name to identify the parameter. Then you need to also set the value for the parameter, this you can say use the default value.}

\textbf{Set Test Oracle}: When retrieving key-value pairs, once the keys \textit{``longitudinal\_oracle''} and \textit{``lateral\_oracle''} are identified, their corresponding values, such as \textit{decelerate} and \textit{keep\_lane}, are obtained and directly fed to the template function \texttt{set\_test\_oracle} to set the scenario monitor.

% The \textit{longitudinal oracle} and \textit{lateral oracle} elements in the scenario representation are directly fed to the template function \texttt{set\_test\_oracle} to set the scenario monitor.\jz{I don't get how you do the set test oracle. Describe how the dictionary looks like and how you map the dictionary to the settestoracle function. I would presume you have two dictionary from the scenario representation. So you assign key Lateraloralce and assign one element such as keep lane as the the value.  Then from the key name, you know it is part of the settestoracle, and you mapp the parameter with the subcomponent name, and assign the parameter value with the element? Can you write in such a way so that reviewer know how you do the dictionary search.  How your dictionary looks like, how you map the dictionary value and key to the function, parameter, and parameter value.  Be clear, I think setoracle and setenvironment might be different? Because settestoracle receives two subcompnents, you can directly set the values for the parameters from elements.  But for setenvironment, not only you need to set the value as foggy which is the element, but you need to provide an normalized value, right? these values are not in the dictionary as they dont' appear in the DSL thus the scenario representation. You need to be very clear about it}

% As our DSL does not ask users to define parameters, in an effort to maintain simplicity in test scenario descriptions, the parameters are assigned default values in the current work. Future work will explore the parameter space using search-based methods to generate a more diverse array of test scenarios that align with traffic rule descriptions.
% \jz{this is confusing, you can simply say in our DSL we don't ask users to define the values for the parameters, for instance if it is rainy, we don't ask the user to specify how hard is the rain.  Then you can say in this work we use the default value from the given simulator and as a future work, we can use search-based method to explore such search space to find more corner cases where the traffic rules will be violated}


\subsubsection{Hierarchical Map-based Route search} 
\label{concrete_function_Search} 
To obtain the accurate coordinates of the ego vehicle and NPC actors, we propose a hierarchical map-based route-search algorithm in the test script generator. 
% \textbf{Set Actors}: 
% \jz{I am thinking maybe a better name is called Hierarchical, right? First we need to use the RoadNetwork and the given map to filter out all those existing routes given in the map which do not satisfy the roadnetwork conditions.  Then we use Ego vehicle information, to find the first route satisfying condition.
% Finally for all other actors,  we can use the ego vehicle route to search for the first route satisfying this actor's condition. Please reorganize your sentence accordingly}
\textit{Waypoints and Routes}: The test script generator first obtains \textit{Waypoints} (coordinates) and \textit{routes} information from the simulator map that is used to generate the test scenario. Specifically, waypoints on all roads in the simulation map are directly obtained by calling the corresponding simulator API, such as \texttt{get\_waypoints} in Carla. Then, \textit{routes} are created by connecting two adjacent waypoints along a road lane, as shown in Figure~\ref{fig:route_scenario} (a). Moreover, route-related information such as length, direction, the connecting routes at the start or end waypoints, the presence of traffic signs on the route, and whether the route traverses an intersection or other types of road are retrieved based on the map information in the simulator. 

% {\color{red}how to select waypoints?}

\textit{Road Network Route Filter}: Based on the key-value pairs of \textit{Road network} subcomponents, the test script generator iteratively checks whether each route contains corresponding subcomponent elements and saves qualified routes in a route list. For example, if the key-value pairs \textit{``road type'': ``intersection'', ``road marker'': ``solid line'', ``traffic signs'': [``speed limit sign'']} is obtained, the test script generator will find all routes that contain solid line and pass through an intersection and a speed limit sign into a route list. The route list is then used to identify the potential ego route to set up the ego vehicle.

\textit{Ego Route identification}: With the generated route list, the test script generator searches the eligible route for the ego vehicle based on key-value pairs of \textit{ego vehicle} subcomponents. For example, if the key-value pairs are \textit{``behavior'': ``go forward'', ``position reference'': ``intersection'', ``position relation'': ``behind''}, the route that straightly crosses an intersection is identified as a potential \texttt{ego route}. A list of potential ego routes is obtained for identifying \texttt{NPC routes}.

\textit{NPC Route identification}: Once a potential ego route is identified, the test script generator further checks its nearby routes to identify the NPC routes that meet the requirements of key-value pairs for each \textit{NPC actor} subcomponent (e.g., another route for going forward and crossing with the \texttt{ego route}). If the eligible NPC routes can be found near the potential ego route, both \texttt{ego route} and \texttt{NPC routes} are formally identified. Otherwise, the identification process for NPC routes is iteratively implemented on all potential \texttt{ego route}. If no valid combination of ego and NPC routes can be found after checking all potential ego routes in the route list, the test script generator will declare that the scenario cannot be generated on the current simulation map.

\textit{Actors coordinate identification}:
The ego vehicle's initial position is set at the start waypoint of the previous connecting route to the ego route, enabling the ADS to accelerate to a steady speed before achieving the  start waypoint of the identified ego route (e.g., the entrance of an intersection) of the test scenario. The ego vehicle's destination is set as the end waypoint of the ego route.  Initial points and destinations for other actors are the start and the end waypoints of their respective routes. An example can be found in Figure~\ref{fig:route_scenario} (b). When all coordinates are identified, they are fed to the template function \texttt{set\_actors}.



% \tz{When reading here, it occurred to me that the current split of this section (template scenario generator and concrete scenario generator) is not very good. You should give a more detailed breakdown. This paragraph definitely talks about something non-trivial and deserve to have a subsection header.}The constraints of the road network and actors are converted to \textit{Waypoints} (coordinates) of the initial positions and destinations of the ego vehicle and NPC actors for controlling their movements. To do this, the scenario generator first constructs \textit{Routes} based on the map information provided by the simulator.
% The conversion is based on the map information provided by the simulator. Specifically, the scenario generator obtains the information of \textit{Waypoints} 
% employs data structures \textit{Waypoint} and \textit{Route} to represent map information from the simulator. 
% A Waypoint is a coordinate of a point on a road line on the map,  while 

% a \textit{route} defines a trajectory from one waypoint to the adjacent waypoint along the road lane, as shown in Figure~\ref{fig:route_scenario} (a). Moreover, a \textit{route} also contains attributes such as length, direction, the presence of traffic signs on the route, and whether the route traverses an intersection. Leveraging the route information, the scenario generator identifies a list of routes that satisfy the constraints of the road network (e.g., \texttt{road type, is, intersection}).

% The scenario generator then iterates over each route in the candidate route list. If a route meets the constraints of the ego vehicle, it is designated as the ego route. Subsequently, the generator iterates over the neighboring routes of the ego route to check whether they fulfill the constraints of other actors, thereby generating a list of NPC routes. The iteration process ends once a combination of the ego route and NPC routes that satisfy all constraints for the ego vehicle and other actors is found. The parameters for the initial and destination positions of all actors are then identified based on the established ego route and NPC routes. The ego vehicle's initial position is set at the starting point of the previous route to the ego route, enabling the ADS to accelerate to a steady speed before achieving the trigger point of the test scenario. The ego vehicle's destination is set as the end waypoint of the ego route.  Initial points and destinations for other actors are the start and the end waypoints of their respective routes. An example can be found in Figure~\ref{fig:route_scenario} (b).

% When API invocations and parameters for all functions are identified, the concrete scenario script is formed for rendering the corresponding scenario.

% Based on the selected routes and the constraints of actors, The scenario generator determines accurate parameters including the initial positions and destinations of actors) for the ego vehicle and other actors. It verifies each route for its compatibility with the behavior constraint, such as turning left, of the ego vehicle. For the eligible route, the generator checks whether adjacent routes of the eligible route meet the requirements of other actors. When the first combinations of routes eligible for all actor constraints are established, the accurate parameters for all actors can be identified. Specifically, the ego vehicle's initial position is set at the starting point of the predecessor route to the ego route, allowing the ADS to reach a steady speed before the test scenario begins. The ego vehicle's destination is the endpoint of the ego route. Spawn points and destinations for other actors are linked directly to their respective routes. An example can be found in Figure~\ref{fig:route_scenario} (b).

% For test oracles, the scenario generator integrates the corresponding test oracle API in accordance with the constraints. For some test orcale APIs, parameters are derived from traffic rule handbooks~\cite{texasDriverHandbook}, such as 3-second safety distance for the longitudinal oracle \textit{keep distance}. In addition, some parameters are derived from the map information. For example, the test oracle \textit{decelerate} checks whether the speed of the ego vehicle decelerates to less than the speed limit specified on the speed limit sign on the road.




% Speed limits are evaluated either by road signs or, in their absence, by comparing average speeds over the route halves. A safe driving distance is maintained using a predefined 3-second parameter from driver handbooks.

% For test oracles, the scenario generator incorporates the corresponding test oracle API such as \texttt{stop}, \texttt{decelerate}, \texttt{keep distance}, and \texttt{keep lane}, according to the constraints. The parameters of the are drawn from traffic rule handbooks~\cite{texasDriverHandbook} and  Speed limits are evaluated either by road signs or, if absent, by comparing average speeds over the route halves. Safe driving distance is maintained using a predefined 3-second parameter from driver handbooks. 
% \\
% \\
% When the four components are constructed, the scenario generator combines them to create the scenario script that can be loaded by the simulator to render the corresponding scenario.

% \subsubsection{Environment Creation}
% Based on elements in the field \textit{Environment} of the scenario representation, the scenario generator invokes corresponding simulator APIs to define the weather in the driving environment. As our DSL does not allow users to define parameters due to the aim of keeping the simple way to describe test scenarios, in the current work, all parameters are assigned as default values. For environment parameters such as \texttt{fog}, the parameter is set as 0.5. In future work, we will explore the parameter space using search-based methods to create more diverse test scenarios in accordance with traffic rule descriptions.

% On the other hand, the scenario generator also controls traffic signals within the simulator. If words related to ``traffic light'' is mentioned in the scenario representation, the scenario generator ensures that the traffic light is in the corresponding status (e.g., red) when the ego vehicle approaches it.


% \begin{figure}[tb!]
% \centering
% \includegraphics[width = .7\textwidth]{image/scenario_example_.pdf}
% \caption{The demonstration of waypoints, routes, and a driving scenario}
% \label{fig:route_scenario}
% \end{figure}


\begin{figure}[tb!]
\centering
\includegraphics[width = .5\textwidth]{image/road.pdf}
\caption{The demonstration of waypoints, routes, and a driving scenario}
\label{fig:route_scenario}
\end{figure}

% \subsubsection{Scenario Location Identification}
% Leveraging on the map information provided by the simulator and elements in the scenario representation, the scenario generator identifies all locations where the test scenario possibly occurs. Specifically, the generator samples waypoints on all lanes in the map and forms routes by connecting adjacent waypoints, as examples shown in Figure~\ref{fig:route_scenario} (a). For each route, its attributes such as length, direction, and whether it crosses an intersection are calculated based on the map information. Then, the generator applies enumerative search to select routes that match the \textit{Road network} elements in the scenario representation, such as selecting all routes that cross an intersection when the element \texttt{intersection} is specified in the \textit{Road network} field.

% During the enumerative search process of routes, the generator also identifies whether the current route is compatible with the behavioral requirements (e.g., turn left) of the ego vehicle and other actors. 

% Based on the selected routes, The scenario generator determines accurate spawn points (i.e., the initial positions of actors) and destinations for both the ego vehicle and other actors based on a depth-first search. It verifies each route for its compatibility with the behavioral requirements of the ego vehicle defined in the scenario representation, like turning left. For the eligible route, the generator checks whether adjacent routes of the eligible route meet the requirements of other actors. When the first combinations of routes eligible for all actors are established, the search process ends, and the generator assigns spawn points and destinations for all actors. The ego vehicle's spawn point is set at the starting point of the predecessor route to the ego route, allowing the ADS to reach a steady speed before the test scenario begins. The ego vehicle's destination is the endpoint of the ego route. Spawn points and destinations for other actors are linked directly to their respective routes. An example can be found in Figure~\ref{fig:route_scenario} (b).


% \subsubsection{Test Oracle Creation}
% \label{sec:test_criteria}
% The scenario generator incorporates various oracle options to determine the expected ego vehicle behavior, such as \texttt{yield}, \texttt{stop}, \texttt{decelerate}, \texttt{keep distance}, and \texttt{keep lane}, according to elements in the field \texttt{Oracle} in the scenario representation. These options, drawn from traffic rule handbooks~\cite{texasDriverHandbook} and OpenXOntology~\cite{openxontology}, assess adherence to right-of-way rules, traffic signs, speed limits, safe driving distances, and lane maintenance. Speed limits are evaluated either by road signs or, if absent, by comparing average speeds over the route halves. Safe driving distance is maintained using a predefined 3-second parameter from driver handbooks. 
% \\
% \\
% When the four components are constructed, the scenario generator combines them to create the scenario script that can be loaded by the simulator to render the corresponding scenario.

